ETAP: Energy-aware Timing Analysis of Intermittent Programs

Energy harvesting battery-free embedded devices rely only on ambient energy harvesting that enables stand-alone and sustainable IoT applications. These devices execute programs when the harvested ambient energy in their energy reservoir is sufficient to operate and stop execution abruptly (and start charging) otherwise. These intermittent programs have varying timing behavior under different energy conditions, hardware configurations, and program structures. This paper presents Energy-aware Timing Analysis of intermittent Programs (ETAP), a probabilistic symbolic execution approach that analyzes the timing and energy behavior of intermittent programs at compile time. ETAP symbolically executes the given program while taking time and energy cost models for ambient energy and dynamic energy consumption into account. We evaluated ETAP on several intermittent programs and compared the compile-time analysis results with executions on real hardware. The results show that ETAP's normalized prediction accuracy is 99.5%, and it speeds up the timing analysis by at least two orders of magnitude compared to manual testing.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> motion_detection_table.tex <==


Variant 1 (ms)
		   100cm		               140cm
meas.	2983.082	142.792	    17,703.459	19.83
0: (1,045)                      0: (17,5)  
1: (6,300)                      1: (18)
etap.	
0: (1,056,026us 19.65572us)     0: (1056026 19.65572) 
1: (1,710,414us 19.75503us)     1: (?us ?us) 


Variant 2 (ms)
		       100cm		            140cm
meas.	6082.200	200.715	  26490.915	624.588
etap.	

0: (?us ?us)    0: (?us ?us) 
1: (?us ?us)    1: (?us ?us) 


CONFIG - 1
Harvesting Time ---------------------

Time @  1MHz  |  100cm  |  50mF  (us)
 Mean Sd
 4,603,800 23361.79 

Time @  1MHz  |  140cm  |  50mF  (us)
 Mean Sd
 16,279,368 5209.22 
 
CONFIG - 2 
Harvesting Time ---------------------

Time @  1MHz  |  100cm  |  50mF  (us)
 Mean Sd
 5066162 18198.48 

Time @  1MHz  |  140cm  |  50mF  (us)
 Mean Sd
 14839892 19277.65 

==> program_transformation.tex <==
\section{Program Transformation: Block-Splitting}
\label{sec:program_transformation}

Program transformation...

==> related_tab.tex <==


\begin{table*}
	\centering
	\scriptsize
	%
	\caption{A comparison of the main features of \sysname with the relevant intermittent computing approaches. \sinan{Ferhat can you modify (or even recreate) this table to have a clear picture where does ETAP stand?} }

	\begin{tabular}{
			>{\centering}m{0.17\textwidth}
			>{\centering}m{0.13\textwidth}
			>{\centering}m{0.07\textwidth}
			>{\centering}m{0.13\textwidth}
			>{\centering}m{0.08\textwidth}
			>{\centering}m{0.08\textwidth}
			>{\centering}m{0.06\textwidth}
			>{\centering}m{0.06\textwidth}
			m{0.17\textwidth}<{\centering}}
		\toprule		

		\multirow{2}{*}{\centering \bf Intermittent Runtimes}
		& \multicolumn{7}{c}{\bf Main Features}  & \multirow{2}{3cm}{\centering \bf Timely, Event-Driven Intermittent Program Development} \\ 
		&  \em Task-based or Checkpointing &
		\em Run-time Overhead &
		\em Event-driven Support  & 		
		\em Cognitive burden &
		\em Lost Work & 	
		\em Local Continuation & 	
		\em Timely Execution & \\
		\midrule
        \rowcolor{black!3} 
		DINO~\cite{dino}, Hibernus++~\cite{hibernus++}, QuickRecall~\cite{quickrecall}, HarvOS~\cite{harvos} & Checkpointing & High \xmark & No Support \xmark & Low \cmark & Low to High \xmark & Yes \cmark & No \xmark  & N/A \xmark \\ 
		
		Ratchet~\cite{ratchet} & 	Checkpointing & Very High \xmark  & No Support \xmark & Low \cmark & Very Low \cmark & Yes \cmark & No \xmark & N/A \xmark \\
		
		\rowcolor{black!3} 
		Chinchilla~\cite{chinchilla} & 	Checkpointing & Medium \xmark  & No Support \xmark &  Low \cmark & Low \cmark & Yes \cmark & No \xmark & N/A \xmark \\ 
		
		Chain~\cite{chain}, 
		Coala~\cite{coala},
		 & 	Task-based & Low \cmark & No Support \xmark & High  \xmark  & High \xmark & No \xmark & No \xmark & N/A \xmark \\
		
		\rowcolor{black!3} 			
		Mayfly~\cite{mayfly} & Task-based & Low \cmark & No Support \xmark & High \xmark & High \xmark & No \xmark & Yes \cmark  & N/A \xmark \\
		
		TICS~\cite{tics} & Checkpointing & Medium \cmark & No Support \xmark & Low \cmark & High \xmark & Yes \cmark & Yes \cmark & N/A \xmark  \\
		
		\rowcolor{black!3} 			
		InK~\cite{ink} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark & High \xmark &  No \xmark & Yes \cmark & Difficult \xmark \\
		
		Coati~\cite{coati} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark & High \xmark &  No \xmark & No \xmark & Difficult \xmark \\
		
		\rowcolor{black!3} 				
		CatNap~\cite{catnap} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark  & High \xmark &  No \xmark & Yes \cmark & Difficult \xmark \\		
		
		\rowcolor{babyblueeyes!25} 
		\textbf{\sysname} \\ (this work) & \textbf{Checkpointing} (almost zero overhead) & \textbf{Low} \cmark & {\bf Full Support} \cmark \\ (all core abstractions) & \textbf{Very Low}  \cmark  & \textbf{Very Low \cmark} (almost zero)  & \textbf{Yes} \cmark & \textbf{Yes} \cmark & \textbf{Easy} \cmark (almost the same as in continuous systems) \\
		\bottomrule
	\end{tabular}
	\label{table:methods_comparison}
\end{table*}

==> related_tab__backup_.tex <==

\setlength{\tabcolsep}{0.15em}   
\newcolumntype{C}[1]{>{\centering}m{#1}}
\begin{table*}
	\centering
	\scriptsize
	%
	\begin{tabular}{
			>{\centering}m{0.17\textwidth}
			>{\centering}m{0.13\textwidth}
			>{\centering}m{0.07\textwidth}
			>{\centering}m{0.13\textwidth}
			>{\centering}m{0.08\textwidth}
			>{\centering}m{0.08\textwidth}
			>{\centering}m{0.06\textwidth}
			>{\centering}m{0.06\textwidth}
			m{0.17\textwidth}<{\centering}}
		\toprule		

		\multirow{2}{*}{\centering \bf Intermittent Runtimes}
		 & \multicolumn{7}{c}{\bf Main Features}  & \multirow{2}{3cm}{\centering \bf Timely, Event-Driven Intermittent Program Development} \\ 
		&  \em Task-based or Checkpointing &
		\em Run-time Overhead &
		\em Event-driven Support  & 		
		\em Cognitive burden &
		\em Lost Work & 	
		\em Local Continuation & 	
		\em Timely Execution & \\
		\midrule
        \rowcolor{black!3} 
		DINO~\cite{dino}, Hibernus++~\cite{hibernus++}, QuickRecall~\cite{quickrecall}, HarvOS~\cite{harvos} & Checkpointing & High \xmark & No Support \xmark & Low \cmark & Low to High \xmark & Yes \cmark & No \xmark  & N/A \xmark \\ 
		
		Ratchet~\cite{ratchet} & Checkpointing & Very High \xmark  & No Support \xmark & Low \cmark & Very Low \cmark & Yes \cmark & No \xmark & N/A \xmark \\
		
		\rowcolor{black!3} 
		Chinchilla~\cite{chinchilla} & 	Checkpointing & Medium \xmark  & No Support \xmark &  Low \cmark & Low \cmark & Yes \cmark & No \xmark & N/A \xmark \\ 
		
		Chain~\cite{chain}, 
		Coala~\cite{coala},
		 & 	Task-based & Low \cmark & No Support \xmark & High  \xmark  & High \xmark & No \xmark & No \xmark & N/A \xmark \\
		
		\rowcolor{black!3} 			
		Mayfly~\cite{mayfly} & Task-based & Low \cmark & No Support \xmark & High \xmark & High \xmark & No \xmark & Yes \cmark  & N/A \xmark \\
		
		TICS~\cite{tics} & Checkpointing & Medium \cmark & No Support \xmark & Low \cmark & High \xmark & Yes \cmark & Yes \cmark & N/A \xmark  \\
		
		\rowcolor{black!3} 			
		InK~\cite{ink} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark & High \xmark &  No \xmark & Yes \cmark & Difficult \xmark \\
		
		Coati~\cite{coati} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark & High \xmark &  No \xmark & No \xmark & Difficult \xmark \\
		
		\rowcolor{black!3} 				
		CatNap~\cite{catnap} & Task-based & Low \cmark & Limited Support \cmarkbad & High \xmark  & High \xmark &  No \xmark & Yes \cmark & Difficult \xmark \\		
		
		\rowcolor{babyblueeyes!25} 
		\textbf{\sysname} \\ (this work) & \textbf{Checkpointing} (almost zero overhead) & \textbf{Low} \cmark & {\bf Full Support} \cmark \\ (all core abstractions) & \textbf{Very Low}  \cmark  & \textbf{Very Low \cmark} (almost zero)  & \textbf{Yes} \cmark & \textbf{Yes} \cmark & \textbf{Easy} \cmark (almost the same as in continuous systems) \\
		\bottomrule
	\end{tabular}
	\caption{A comparison of the main features of \sysname with the relevant intermittent computing approaches. \sinan{Ferhat can you modify (or even recreate) this table to have a clear picture where does ETAP stand?} }
	\label{table:methods_comparison}
\end{table*}

==> related_table.tex <==
\begin{table}%[!ht]
\centering
  \footnotesize
  \caption{A comparison of the main features of \sysname with the relevant intermittent computing approaches.}
  \label{tab:related-table}
  \begin{tabularx}{\linewidth}{@{}XXXXX@{}} 
  \toprule
\multicolumn{1}{c}{\bf System}   &\multicolumn{1}{c}{Analysis}   &\multicolumn{1}{c}{Timing}   &\multicolumn{1}{c}{Energy}   &\multicolumn{1}{c}{Analysis}\\
                  {}                               &{Type}                    &{Analysis}                   &{Analysis}                   &{Precision}\\
\midrule
  \rowcolor{black!3} 
EPIC~\cite{epic}         &Runtime &No Support \xmark &Yes \cmark & \\
CleanCut~\cite{cleancut} &Runtime &No Support \xmark &Yes \cmark  & \\
   \rowcolor{black!3}                    
Siren~\cite{siren}       & &No Support \xmark & & \\
Ocelot~\cite{ocelot}     & &No Support \xmark & & \\
   \rowcolor{black!3}                    
TICS~\cite{tics}         & &No Support \xmark & & \\
Mayfly~\cite{mayfly}     & &No Support \xmark & & \\
   \rowcolor{black!3}                    
Samoyed~\cite{samoyed}   & &No Support \xmark & & \\
Zygarde~\cite{zygarde}   & &No Support \xmark & & \\
   \rowcolor{black!3}                    
% CatNap~\cite{catnap}     & &No Support  \xmark & & \\
% PREAcT~\cite{preact}     & &No Support \xmark & & \\
   % \rowcolor{black!3}                    
% CHRT~\cite{chrt}         & &No Support \xmark & & \\
\rowcolor{babyblueeyes!25}
\textbf{\sysname}        &\textbf{Compile-Time} &\textbf{Yes} \cmark &\textbf{Yes} \cmark  &\textbf{High} \\
\bottomrule
  \end{tabularx}
\end{table}
